The Complexity of Dynamic Data Race Prediction

Writing concurrent programs is notoriously hard due to scheduling non-determinism. The most common concurrency bugs are data races, which are accesses to a shared resource that can be executed concurrently. Dynamic data-race prediction is the most standard technique for detecting data races: given an observed, data-race-free trace $t$, the task is to determine whether $t$ can be reordered to a trace $t^*$ that exposes a data-race. Although the problem has received significant practical attention for over three decades, its complexity has remained elusive. In this work, we address this lacuna, identifying sources of intractability and conditions under which the problem is efficiently solvable. Given a trace $t$ of size $n$ over $k$ threads, our main results are as follows. First, we establish a general $O(k\cdot n^{2\cdot (k-1)})$ upper-bound, as well as an $O(n^k)$ upper-bound when certain parameters of $t$ are constant. In addition, we show that the problem is NP-hard and even W[1]-hard parameterized by $k$, and thus unlikely to be fixed-parameter tractable. Second, we study the problem over acyclic communication topologies, such as server-clients hierarchies. We establish an $O(k^2\cdot d\cdot n^2\cdot \log n)$ upper-bound, where $d$ is the number of shared variables accessed in $t$. In addition, we show that even for traces with $k=2$ threads, the problem has no $O(n^{2-\epsilon})$ algorithm under Orthogonal Vectors. Since any trace with 2 threads defines an acyclic topology, our upper-bound for this case is optimal wrt polynomial improvements for up to moderate values of $k$ and $d$. Finally, we study a distance-bounded version of the problem, where the task is to expose a data race by a witness trace that is similar to $t$. We develop an algorithm that works in $O(n)$ time when certain parameters of $t$ are constant.

==> automata.tex <==
\section{Checking Correct Reorderings Against Regular Automata}

\subsection{Upper bounds}

\smallskip
\begin{restatable}{theorem}{them:automataub}\label{them:automata_ub}
Given a finite automata $\Automata$ and a trace ideal $X$, deciding whether $(X,\Automata)$ is realizable can be done in $O(n^k)$ time, for $k$ threads.
\end{restatable}

\subsection{Lower bounds}


\begin{restatable}{lemma}{lem2threadslb}\label{lem:2threads_lb}
Consider a trace $\Trace$ of $k=2$ threads and a regular automata $\Automata$.
Let $X$ be a trace ideal of $\Trace$ such that $X$ contains $n_i$ events from thread $i$.
There exists no algorithm for the realizability of $(X,\Automata)$ that operates in time $O(n_1^{1-\delta}\cdot n_2^{1-\epsilon})$ for any $\epsilon, \delta \geq 0$ such that $\epsilon\cdot \delta >0$,
unless the Orthogonal Vectors conjecture fails.
\end{restatable}
\begin{proof}[Sketch]
For a fine-grained reduction from Orthogonal Vectors, consider an instance $(A,B)$ of the Orthogonal Vectors problem where each set contains $n/2$ vectors of dimension $d$.
We construct two alphabets $\Sigma_1=\{ 0,1,\# \}$ and $\Sigma_2={ 2 }$ and an independence relation $\Independence=\Sigma_1\times \Sigma_2$.
We construct a trace ideal that consists of two threads $\Process_1, \Process_2$, such that $\Process_i$ contains events of $\Sigma_i$.
In particular, the sequential trace of  $\Process_1$ has the form $\SeqTrace_1=a_1\#\dots a_{n/2}\#\#b_1\#\dots b_{n/2}\#$,
where $a_i$ and $b_i$ range over the vectors of $A$ and $B$, respectively.
The sequential trace of $\Process_2$ contains the string $\SeqTrace_2=2^n$.
Note that the two traces have lengths $O(n\cdot d)$ and $n/2$, respectively.

We will now describe an alternating automata $\Automata$ such that $(X,\Automata)$ is realizable iff there exist $i,j\in [n/2]$ such that $a_i$ is orthogonal to $b_j$.
The automata $\Automata$ initially scans only events of $\Trace_1$, and when encountering the delimiter $\#$, it non-deterministically decides that $\#$ marks the beginning of the vector $a$.
Then, $\Automata$ enters a $\forall$ state, in which it reads letters of $\SeqTrace_1$ and $\SeqTrace_2$ alternatingly, until it decides to check the product of the $\ell$-th bit of $a$ against the $\ell_1$-th bit of the second vector $b$ (to be chosen in the future).
At this point $\Automata$ stops reading from $\SeqTrace_2$, and it reads from $\SeqTrace_1$ until it encounters $\#\#$.
Then it keeps reading from $\SeqTrace_1$ until, when encountering $\#$, it decides that the symbol marks the beginning of the second vector $b$.
It then keeps reading from $\SeqTrace_1$ until it non-deterministically chooses a bit $\ell_2$ of $b$.
If $a[\ell_1] \cdot b[\ell_2]=0$, then $\Automata$ accepts.
Otherwise, $\Automata$ starts reading alternatingly in $\SeqTrace_1$ and $\SeqTrace_2$.
If the symbol $\#$ is encountered in $\SeqTrace_1$ when all of $\SeqTrace_2$ has been read, then $\Automata$ rejects, otherwise it accepts.

Let $n_1=|\SeqTrace_1|=O(n\cdot d)$ and $n_2=|\SeqTrace_2|=n$, and assume that the realizability of $(X, \Automata)$ can be decided in time $O(n_1^{1-\delta}\cdot n_2^{1-\epsilon})$ for some $\epsilon, \delta \geq 0$ such that $\epsilon\cdot \delta >0$.
Then the Orthogonal Vectors instance is solved in time
\[
(n\cdot d)^{1-\epsilon}\cdot n^{1-\delta} = n^{2-\epsilon-\delta+\epsilon\cdot \delta}\cdot d^{1-\epsilon} \numberthis\label{eq:ov}
\]
If $\delta>0$, note that the exponent of $n$ is $<2$ since $\epsilon < 1$ and thus $\delta > \delta\cdot \epsilon$.
Similarly for $\epsilon>0$.
\end{proof}

\Andreas{The above should yield a general result for all $k\geq 2$.}


==> closed_partial_orders.tex <==
\section{Trace-closed Partial Orders}\label{SEC:PO}




==> constant_context_switches.tex <==
\subsection{Constant Context Switches}\label{subsec:constant_context_switches}


\smallskip
\begin{restatable}{theorem}{themconstantcontextswitches}\label{them:constant_context_switches}
Consider a concurrent trace $\Trace$ over $k=O(1)$ threads and $O(1)$ context switches.
Let $\Event_1, \Event_2\in \Events{\Trace}$ be two events of $\Trace$.
Whether $(\Event_1, \Event_2)$ is a predictable data race of $\Trace$ can be decided in $O(n)$ time.
\end{restatable}

==> constant_remote_reads.tex <==
\subsection{Constant Remote Reads}\label{subsec:constant_remote_reads}

\smallskip\noindent{\bf Local triplets and unique reads.}
A read event $\Read$ is said to be \emph{local} if $\Proc{\Read}=\Proc{\Observation_{\Trace}(\Read)}$.
If $\Read$ is not remote then it is \emph{remote}.
Consider a trace ideal $X$ of $\Trace$.
A triplet $(\Write, \Read, \Write')$ of $X$ is called \emph{local} (resp., \emph{remote}) if $\Read$ is local (resp., remote).
A triplet $(\Write, \Read, \Write')$ is called unique in  a trace ideal $X$ if for every triplet $(\Write, \Read, \Write'')$ in $X$ we have $\Write'=\Write''$.
A set of triplets $\{(\Write_i, \Read_i, \Write'_i)\}_i$ is said to be of the \emph{local} if every triplet is local and $\Proc{\Read_i}=\Proc{\Read_j}$ for all $i\neq j$.
We assume w.l.o.g. that every triplet is unique in $\Events{\Trace}$.
A set of triplets $\{(\Write_i, \Read_i, \Write'_i)\}_i$ is said to be of the \emph{fully local}
if it is local and $\Proc{\Write'_i}=\Proc{\Write'_j}$ for each $i\neq j$.



\smallskip
\begin{restatable}{lemma}{lemsamethreadtriplets}\label{lem:same_thread_triplets}
In any local set of at least $k+1$ triplets $\{\sigma_i=(\Write_i, \Read_i, \Write'_i)\}_i$ there exist $i\neq j$ such that 
the set $\{ \sigma_i, \sigma_j \}$ is fully local.
\end{restatable}
\begin{proof}
Follows from the pigeonhole principle.
\end{proof}




\smallskip\noindent{\bf Effective frontiers.}
Let $X$ be a feasible trace ideal of $\Trace$, and $Y$ an ideal of the canonical partially ordered set $(X,P)$.
The \emph{effective frontier} of $Y$, denoted $\EffFrontier{X}{P}{Y}$ is the set of triplets $\sigma_i=(\Write_i, \Read_i, \Write_i')$ over $X$ such that the following conditions hold.
\begin{compactenum}
\item $\sigma_i\in \Frontier{X}{P}{Y}$.
\item There exists no triplet $\sigma_j\in \Frontier{X}{P}{Y}$ such that
the set $\{ \sigma_i, \sigma_j \}$ is fully local and $\Write'_j<_{\TO}\Write'_i$.
\end{compactenum}

\smallskip
\begin{restatable}{lemma}{lemeffectivefrontier}\label{lem:effective_frontier}
Consider a feasible trace ideal $X$ and an ideal $Y$ of the partially ordered set $(X,P)$.
Let $\Event$ be an event enabled in $Y$.
Then $Y$ is extensible with $\Event$ iff there exists no triplet $(\Write_i,\Read_i,\Event)\in \EffFrontier{X}{P}{Y}$.
\end{restatable}
\begin{proof}
Since $\EffFrontier{X}{P}{Y}\subseteq \Frontier{X}{P}{Y}$, if there exists such a triplet then $Y$ is not extensible with $\Event$.
For the inverse direction, assume towards contradiction otherwise.
Hence, there exists a triplet $(\Write_i,\Read_i,\Event)\in \Frontier{X}{P}{Y}$.
Since $(\Write_i,\Read_i,\Event)\not \in \EffFrontier{X}{P}{Y}$, there exists a triplet 
$(\Write_j, \Read_j, \Write'_j)\in \EffFrontier{X}{P}{Y}$ such that the set
$\{(\Write_i,\Read_i,\Event), (\Write_j, \Read_j, \Write'_j)\}$ is fully local and $\Write'_j<{\TO}\Event$.
But then $\Event$ is not enabled in $Y$, a contradiction.

The desired result follows.
\end{proof}


\smallskip
\begin{restatable}{lemma}{lemeffectivefrontiersize}\label{lem:effective_frontier_size}
$|\EffFrontier{X}{P}{Y}|\leq k^2$.
\end{restatable}
\begin{proof}
Every set of $k^1$ + 1 triplets has two triplets that are fully local,
and at most one of them can be in $\EffFrontier{X}{P}{Y}$.
\end{proof}


\smallskip
\begin{restatable}{lemma}{lemidealrealizabilityconstantremotereads}\label{lem:ideal_realizability_constant_remote_reads}
Consider a trace $\Trace$ over $k$ threads and $c$ variables, as well as an ideal $X$ of $\Trace$.
The realizability problem of $X$ can be decided in $O(n\cdot k^{k^2+1})$ time.
\end{restatable}
\begin{proof}
The proof is similar to \cref{lem:ideal_realizability_constant_vars}.
The only difference is that the DFS tree has the property that in every path from the root to a leaf,
there exist at most $k^2$ nodes that are not unary.
\end{proof}


\smallskip
\begin{restatable}{theorem}{themconstantremotereads}\label{them:constant_remote_reads}
Consider a concurrent trace $\Trace$ over $k=O(1)$ threads and $O(1)$ remote read events.
Let $\Event_1, \Event_2\in \Events{\Trace}$ be two events of $\Trace$.
Whether $(\Event_1, \Event_2)$ is a predictable data race of $\Trace$ can be decided in $O(n)$ time.
\end{restatable}
\begin{proof}
{\bf AP: I might have to assume constant locks as well.}
\end{proof}


==> constant_variables.tex <==
\subsection{Constant Variables}\label{subsec:constant_variables}

\smallskip\noindent{\bf Frontier locations.}
Given a trace $\Trace$, an ideal $X$ of $\Trace$, and a set $Y\subseteq X$, the \emph{location frontier} of $Y$, denoted by $\LocFrontier{X}{Y}$, is defined as
\[
\LocFrontier{X}{Y}=\{ \Location{\Write}\colon \exists (\Write, \Read)\in\Frontier{\Events{\Trace}}{X} \}
\]
i.e., it is the set of locations of the frontier of $X$.
To simplify notation, we extend the notion of frontier locations to correct reorderings of $\Trace$, 
so that given a correct reordering $\Trace'$ of $\Trace$ with $\Events{\Trace'}\subseteq X$, we have
$\LocFrontier{X}{\Trace'}=\LocFrontier{X}{\Events{\Trace'}}$.



\smallskip
\begin{restatable}{lemma}{lemexecutionpaths}\label{lem:execution_paths}
Consider the trace space $\Tree_X=(\TreeNodes_X, \TreeEdges_X, \Label_X)$
and two traces $\Trace_1, \Trace_2\in \TreeNodes_X$ such that
$\Trace_1$ is an ancestor of $\Trace_2$ and $\LocFrontier{X}{\Trace_2}\subseteq \LocFrontier{X}{\Trace_1}$.
Then $\Trace_1$ is accepting iff $\Trace_2$ or some $\Trace'\in \Ancestors{X}{\Trace_2}\cap \Descendants{X}{\Trace_1}$ is accepting.
\end{restatable}
\begin{proof}
If some descendant of $\Trace_1$ is accepting then clearly $\Trace_1$ is accepting.
Here we focus on the inverse direction, i.e., if $\Trace_1$ is accepting, then $\Trace_2$ or some $\Trace'\in \Ancestors{X}{\Trace_2}\cap \Descendants{X}{\Trace_1}$ is accepting.
The statement holds trivially if $\Trace_1$ is a unary node, hence we assume that $\Trace_1$ is not unary.
By construction, every child of $\Trace_1$ has the form $\Trace_1^{\Write_i}=\Trace_1\circ \Write_i$, 
such that there is a pair $(\Write_i, \Read_i)\in \Frontier{X}{\Events{\Trace_1}}$.
Assume wlog that $\Trace_1^{\Write_1}\in \Ancestors{X}{\Trace_2}$, and the statement follows easily if $\Trace_1^{\Write_1}$ is accepting.

\end{proof}






\smallskip
\begin{restatable}{lemma}{lemidealrealizabilityconstantvars}\label{lem:ideal_realizability_constant_vars}
Consider a trace $\Trace$ over $k$ threads and $c$ variables, as well as an ideal $X$ of $\Trace$.
The realizability problem of $X$ can be decided in $O(n\cdot k^{c+1})$ time.
\end{restatable}
\begin{proof}
Indeed, consider a simple algorithm that traverses $G_X=(V_X, E_X)$ as follows.
We start from $\emptyset$ and perform a DFS. 
Given the current ideal $Y$, if $Y$ has a child $Z$ such that $\Location{Y} \not \subseteq \Location{Z}$, then we proceed to $Z$ and never examine any other child of $Y$.

The correctness of the algorithm follows directly from \cref{lem:execution_paths}.
To reason about the complexity, consider the DFS tree $\Tree=(\TreeNodes, \TreeEdges)$ traversed by the algorithm.
In every path from the root to a leaf we have at most $c$ non-unary nodes.
By \cref{lem:thin_tree}, we have $|\TreeNodes|\leq n\cdot k^c$.
Since in every node of $\Tree$ we perform $O(k)$ operations, the desired result follows.
\end{proof}



\smallskip
\begin{restatable}{theorem}{themconstantthreads}\label{them:constant_variables}
Consider a concurrent trace $\Trace$ over $k=O(1)$ threads and $c=O(1)$ variables.
Let $\Event_1, \Event_2\in \Events{\Trace}$ be two events of $\Trace$.
Whether $(\Event_1, \Event_2)$ is a predictable data race of $\Trace$ can be decided in $O(n)$ time.
\end{restatable}
\begin{proof}
We argue that it suffices to test $O(1)$ feasible trace ideals $X$ in which $\Event_1, \Event_2$ are enabled,
as then the statement follows from \cref{lem:ideal_realizability_constant_vars}.
Indeed, for any two feasible trace ideals $X$ and $Y$, such that $\Event_1, \Event_2$ are enabled in both $X$ and $Y$, if $\OpenLockMap_X=\OpenLockMap_Y$, by \cref{lem:constant_ideals}, it suffices to only test one of them.
Hence it suffices to test as many feasible trace ideals as different open-lock maps.
Observe that we have at most
\begin{align}
\left(k+1\right)^{|\Locks|} \leq (k+1)^c=O(1)
\end{align}
many open-lock maps.

The desired result follows.
\end{proof}

==> figures/fig_race_reduction.tex <==
\begin{figure}
\newcommand{\xdisposition}{0}
\newcommand{\ydisposition}{0}
\newcommand{\xtstep}{0.9}
\newcommand{\ytstep}{0.5}
\newcommand{\xstep}{2.8}
\newcommand{\ystep}{1.2}
\newcommand{\xtscale}{0.75}

\def \mycolone {black!20!green}
\def \mycoltwo {black!20!blue}
\def \mycolthree {black!20!orange}
\def \mycolfour {black!20!red}
\def \mycolfive {black!20!black}

\def \mycolone {black}
\def \mycoltwo {black}
\def \mycolthree {black}
\def \mycolfour {black}
\def \mycolfive {black}

%Arguments are name prefix, color, x,y
\newcommand{\drawtriplet}[4]{
\node[] (w#1) at (#3,#4)  {$\textcolor{#2}{\Write_{#1}}$};
\node[] (r#1) at (#3,#4-2*\ytstep)  {$\textcolor{#2}{\Read_{#1}}$};
\node[] (wp#1) at (#3+\xtscale*\xtstep,#4-1*\ytstep)  {$\textcolor{#2}{\Write'_{#1}}$};
}
\newcommand{\drawtripletR}[4]{
\node[] (w#1) at (#3+\xtscale*\xtstep,#4)  {$\textcolor{#2}{\Write_{#1}}$};
\node[] (r#1) at (#3+\xtscale*\xtstep,#4-2*\ytstep)  {$\textcolor{#2}{\Read_{#1}}$};
\node[] (wp#1) at (#3,#4-1*\ytstep)  {$\textcolor{#2}{\Write'_{#1}}$};
}
\begin{subfigure}[b]{0.45\textwidth}
\centering
\begin{tikzpicture}[thick,
pre/.style={<-,shorten >= 2pt, shorten <=2pt, very thick},
post/.style={->,shorten >= 2pt, shorten <=2pt,  very thick},
seqtrace/.style={->, line width=2},
und/.style={very thick, draw=gray},
event/.style={rectangle, minimum height=0.8mm, minimum width=3mm, fill=black!100,  line width=1pt, inner sep=0},
virt/.style={circle,draw=black!50,fill=black!20, opacity=0}]





\drawtriplet{1}{\mycolone}{0*\xstep}{0*\ystep}
\drawtripletR{2}{\mycoltwo}{1*\xstep}{0*\ystep}
\draw[->, thick] (wp2) to (wp1);

\node[] at (0.5*\xstep,-2*\ystep) {$
\Trace=\textcolor{\mycolfour}{\Write'_2}\textcolor{\mycolfive}{\Write'_1}
\textcolor{\mycolone}{\Write_1}\textcolor{\mycoltwo}{\Write_2}
\textcolor{\mycolone}{\Read_1}\textcolor{\mycoltwo}{\Read_2}
$};

\node[] at (0.5*\xstep,-2.5*\ystep) {$\sigma=(\Write_2, \Read_2, \Write'_2)$};

%\node[] at(0,-8*\ytstep) {};

\end{tikzpicture}
\caption{
An instance of $\ROPosetRealizability$.
}
\label{subfig:race_reduction1}
\end{subfigure}
\begin{subfigure}[b]{0.45\textwidth}
\centering
\footnotesize
\def\rownumber{}
\begin{tabular}[b]{@{\makebox[1.2em][r]{\rownumber\space}} | l | l | l | l |}
\normalsize{$\mathbf{\SeqTrace_1}$} & \normalsize{$\mathbf{\SeqTrace_2}$} & \normalsize{$\mathbf{\SeqTrace_3}$} & \normalsize{$\mathbf{\SeqTrace_4}$}
\gdef\rownumber{\stepcounter{magicrownumbers}\arabic{magicrownumbers}} \\
\hline
& & & $\Acquire(\ell)$\\
& & & $\Write'(x_2)$ \\
& & & $\Write(x_{\Write'_2, \Write'_1})$\\
& & & $\mathbf{\ov{\Write}(y)}$\\
& & & $\Release(\ell)$\\
& & $\Read(x_{\Write'_2, \Write'_1})$ & \\
& & $\Write'(x_1)$ & \\
& & $\Write(x^2)$ &  \\
&  $\Write(x_2)$ & &\\
&  $\Acquire(\ell)$ & & \\
&  $\Read(x_2)$ & & \\
&  $\Release(\ell)$ & & \\
$\Write(x_1)$ & & & \\
$\Read(x_1)$ & & & \\
$\Write(x^1)$ & & & \\
& $\Read(x^1)$ & &\\
& $\Read(x^2)$ & &\\
& $\mathbf{\ov{\Read}(y)}$ & &\\
\hline
\end{tabular}
\caption{The instance of race prediction using our reduction.}
\label{subfig:race_reduction2}
\end{subfigure}
\caption{
Example of our reduction of an instance of $\ROPosetRealizability$ (\protect\ref{subfig:race_reduction1}) to an instance of race prediction (\protect\ref{subfig:race_reduction2}), where the task is to decide whether $(\Event_{4}, \Event_{18})$ is a predictable race of the input trace.
}
\label{fig:race_reduction}
\end{figure}


==> figures/fig_reverseA.tex <==
\begin{figure}
\newcommand{\xdisposition}{0}
\newcommand{\ydisposition}{0}
\newcommand{\xtstep}{0.5}
\newcommand{\ytstep}{0.5}
\newcommand{\xstep}{1.5}
\newcommand{\ystep}{-0.8}
\newcommand{\xtscale}{0.8}

\def \mycolone {blue}
\def \mycoltwo {green!70}
\def \mycolthree {yellow}
\def \mycolfour {red}
\def \mycolfive {orange}
\def \mycolsix {purple}
\def \mycolseven {magenta}

\def \mycolone {black}
\def \mycoltwo {black}
\def \mycolthree {black}
\def \mycolfour {black}
\def \mycolfive {black}
\def \mycolsix {black}
\def \mycolseven {black}

\def \numevents{9}

%\newcommand{\eventA}[4]{
%\node[event] (#1) at (#2, #3) {};
%\node[] at (#2-\xtstep, #3) {\small #4};
%}
%\newcommand{\eventB}[4]{
%\node[event] (#1) at (#2, #3) {};
%\node[] at (#2+\xtstep, #3) {\small #4};
%}

\newcommand{\event}[4]{
\node[event] (#1) at (#2, #3) {\small #4};
}

\begin{tikzpicture}[thick,
pre/.style={<-,shorten >= 2pt, shorten <=2pt, very thick},
post/.style={->,shorten >= 2pt, shorten <=2pt,  very thick},
seqtrace/.style={->, line width=2},
node/.style={circle, draw=black, inner sep=2pt, line width=1pt},
und/.style={very thick, draw=gray},
event/.style={rectangle, minimum height=0.8mm, minimum width=5mm,  line width=1pt, inner sep=1.5, fill=white, draw=black},
virt/.style={circle,draw=black!50,fill=black!20, opacity=0}]

\begin{scope}[shift={(-2.5,2*\ystep)}]
\node[] at (0.5,1) {$G$};
\node[node] (1) at (0,0) {$1$};
\node[node] (2) at (1,0) {$2$};
\node[node] (3) at (0,-1) {$3$};
\node[node] (4) at (1,-1) {$4$};
\draw[-, very thick] (3) to (1);
\draw[-, very thick] (3) to (2);
\end{scope}

\node[] (SW1A) at (0*\xstep,0) {$\SeqTrace_{1}$};
\node[] (SW1B) at (0*\xstep,\numevents * \ystep) {};
\node[] (SW2A) at (1*\xstep,0) {$\SeqTrace_{2}$};
\node[] (SW2B) at (1*\xstep,\numevents * \ystep) {};
\node[] (SW3A) at (2*\xstep,0) {$\SeqTrace_{3}$};
\node[] (SW3B) at (2*\xstep,\numevents * \ystep) {};

\draw[seqtrace] (SW1A) to (SW1B);
\draw[seqtrace] (SW2A) to (SW2B);
\draw[seqtrace] (SW3A) to (SW3B);

%\node[] (SR1A) at (\xdisposition +0*\xstep,0) {$\SeqTrace^{\Read}_{1}$};
%\node[] (SR1B) at (\xdisposition +0*\xstep,\numevents * \ystep) {};
%\node[] (SR2A) at (\xdisposition +1*\xstep,0) {$\SeqTrace^{\Read}_{2}$};
%\node[] (SR2B) at (\xdisposition +1*\xstep,\numevents * \ystep) {};
%\node[] (SR3A) at (\xdisposition +2*\xstep,0) {$\SeqTrace^{\Read}_{3}$};
%\node[] (SR3B) at (\xdisposition +2*\xstep,\numevents * \ystep) {};


\event{aw11}{0*\xstep}{1*\ystep}{$\AtomicWrite^{1}_{1}$}
\event{aw12}{0*\xstep}{3*\ystep}{$\AtomicWrite^{1}_{2}$}
\event{aw13}{0*\xstep}{5*\ystep}{$\AtomicWrite^{1}_{3}$}
\event{aw14}{0*\xstep}{7*\ystep}{$\AtomicWrite^{1}_{4}$}

\event{aw21}{1*\xstep}{1*\ystep}{$\AtomicWrite^{2}_{1}$}
\event{aw22}{1*\xstep}{3*\ystep}{$\AtomicWrite^{2}_{2}$}
\event{aw23}{1*\xstep}{5*\ystep}{$\AtomicWrite^{2}_{3}$}
\event{aw24}{1*\xstep}{7*\ystep}{$\AtomicWrite^{2}_{4}$}

\event{aw31}{2*\xstep}{1*\ystep}{$\AtomicWrite^{3}_{1}$}
\event{aw32}{2*\xstep}{3*\ystep}{$\AtomicWrite^{3}_{2}$}
\event{aw33}{2*\xstep}{5*\ystep}{$\AtomicWrite^{3}_{3}$}
\event{aw34}{2*\xstep}{7*\ystep}{$\AtomicWrite^{3}_{4}$}




\event{ar11}{\xdisposition +0*\xstep}{2*\ystep}{$\AtomicRead^{1}_{1}$}
\event{ar12}{\xdisposition +0*\xstep}{4*\ystep}{$\AtomicRead^{1}_{2}$}
\event{ar13}{\xdisposition +0*\xstep}{6*\ystep}{$\AtomicRead^{1}_{3}$}
\event{ar14}{\xdisposition +0*\xstep}{8*\ystep}{$\AtomicRead^{1}_{4}$}

\event{ar21}{\xdisposition +1*\xstep}{2*\ystep}{$\AtomicRead^{2}_{1}$}
\event{ar22}{\xdisposition +1*\xstep}{4*\ystep}{$\AtomicRead^{2}_{2}$}
\event{ar23}{\xdisposition +1*\xstep}{6*\ystep}{$\AtomicRead^{2}_{3}$}
\event{ar24}{\xdisposition +1*\xstep}{8*\ystep}{$\AtomicRead^{2}_{4}$}

\event{ar31}{\xdisposition +2*\xstep}{2*\ystep}{$\AtomicRead^{3}_{1}$}
\event{ar32}{\xdisposition +2*\xstep}{4*\ystep}{$\AtomicRead^{3}_{2}$}
\event{ar33}{\xdisposition +2*\xstep}{6*\ystep}{$\AtomicRead^{3}_{3}$}
\event{ar34}{\xdisposition +2*\xstep}{8*\ystep}{$\AtomicRead^{3}_{4}$}

\draw[->,  thick, ] (aw14) to (aw22);
\draw[->,  thick, ] (aw22) to (aw31);

\draw[->,  thick, ] (ar22) to (ar14);
\draw[->,  thick, ] (ar31) to (ar22);



\draw[->,  thick, ] (ar14) to (aw32);
\draw[->,  thick, ] (ar21) to (aw11);
\draw[->,  thick, ] (ar33) to (aw23);
\draw[->,  thick, ] (ar23) to (aw34);
\draw[->,  thick, ] (ar34) to (aw24);

%\draw[->,  thick, ] (ar21) to (ar11);
%\draw[->,  thick, ] (ar33) to (ar23);
%\draw[->,  thick, ] (ar23) to (ar34);
%\draw[->,  thick, ] (ar34) to (ar24);
%\draw[->,  thick, bend left=25, ] (ar13) to (ar31);
%\draw[->,  thick, bend left=25, ] (ar14) to (ar32);

\end{tikzpicture}
\caption{
}
\label{fig:reverseA}
\end{figure}

==> figures/fig_rscrm_reduction.tex <==
\begin{figure}
\newcommand{\xdisposition}{0}
\newcommand{\ydisposition}{0}
\newcommand{\xtstep}{0.9}
\newcommand{\ytstep}{0.5}
\newcommand{\xstep}{2.8}
\newcommand{\ystep}{1.2}
\newcommand{\xtscale}{0.8}

\def \mycolone {black!20!green}
\def \mycoltwo {black!20!blue}
\def \mycolthree {black!20!orange}
\def \mycolfour {black!20!red}
\def \mycolfive {black!20!black}

\def \mycolone {black}
\def \mycoltwo {black}
\def \mycolthree {black}
\def \mycolfour {black}
\def \mycolfive {black}

%Arguments are name prefix, color, x,y
\newcommand{\drawtriplet}[6]{
\node[] (w#1) at (#4,#5)  {$\textcolor{#3}{\Write_{#2}}$};
\node[] (r#1) at (#4,#5-2*\ytstep)  {$\textcolor{#3}{\Read_{#2}}$};
\node[] (wp#1) at (#4+\xtscale*\xtstep,#5-1*\ytstep)  {$\textcolor{#3}{\Write'_{#2}}$};
\ifthenelse{#6=1}{\draw[->, thick] (w#1) to (r#1);}{}
}
\newcommand{\drawtripletR}[6]{
\node[] (w#1) at (#4+\xtscale*\xtstep,#5)  {$\textcolor{#3}{\Write_{#2}}$};
\node[] (r#1) at (#4+\xtscale*\xtstep,#5-2*\ytstep)  {$\textcolor{#3}{\Read_{#2}}$};
\node[] (wp#1) at (#4,#5-1*\ytstep)  {$\textcolor{#3}{\Write'_{#2}}$};
\ifthenelse{#6=1}{\draw[->, thick] (w#1) to (r#1);}{}
}
\newcommand{\drawtripletdistinguished}[6]{
\node[] (w#1) at (#4,#5)  {$\textcolor{#3}{\ov{\Write}_{#2}}$};
\node[] (r#1) at (#4,#5-2*\ytstep)  {$\textcolor{#3}{\ov{\Read}_{#2}}$};
\node[] (wp#1) at (#4+\xtscale*\xtstep,#5-1*\ytstep)  {$\textcolor{#3}{\ov{\Write}'_{#2}}$};
\ifthenelse{#6=1}{\draw[->, thick] (w#1) to (r#1);}{}
}
\begin{subfigure}[b]{0.5\textwidth}
\centering
\begin{tikzpicture}[thick,
pre/.style={<-,shorten >= 2pt, shorten <=2pt, very thick},
post/.style={->,shorten >= 2pt, shorten <=2pt,  very thick},
seqtrace/.style={->, line width=2},
und/.style={very thick, draw=gray},
event/.style={rectangle, minimum height=0.8mm, minimum width=3mm, fill=black!100,  line width=1pt, inner sep=0},
virt/.style={circle,draw=black!50,fill=black!20, opacity=0}]


\drawtriplet{1}{1}{\mycolone}{0*\xstep}{0*\ystep}{1}
\drawtripletR{2}{2}{\mycoltwo}{1*\xstep}{0*\ystep}{1}
\draw[->, thick] (wp2) to (wp1);
\draw[->, thick] (r1) to (r2);

%\node[] at(0,-6*\ytstep) {};

\end{tikzpicture}
\caption{
An instance of $\OPosetRealizability$.
}
\label{subfig:rscrm_reduction1}
\end{subfigure}
\begin{subfigure}[b]{0.5\textwidth}
\centering
\begin{tikzpicture}[thick,
pre/.style={<-,shorten >= 2pt, shorten <=2pt, very thick},
post/.style={->,shorten >= 2pt, shorten <=2pt,  very thick},
seqtrace/.style={->, line width=2},
und/.style={very thick, draw=gray},
event/.style={rectangle, minimum height=0.8mm, minimum width=3mm, fill=black!100,  line width=1pt, inner sep=0},
virt/.style={circle,draw=black!50,fill=black!20, opacity=0}]

\begin{scope}[shift={(-3,0)}]
\drawtriplet{1}{1}{\mycolone}{0*\xstep}{0*\ystep}{1}
\drawtripletR{2}{2}{\mycoltwo}{2*\xstep}{0*\ystep}{1}
\drawtriplet{3}{\Read_{1},\Read_{2}}{\mycolthree}{0*\xstep}{-2*\ystep}{1}
\drawtripletR{4}{\Write'_{2},\Write'_{1}}{\mycolfour}{2*\xstep}{-2*\ystep}{1}
\drawtripletdistinguished{5}{}{\mycolfive}{1*\xstep}{-1*\ystep}{1}
\end{scope}

\draw[->, thick, bend right=30] (r1) to (r3);
\draw[->, thick, bend right=20] (wp3) to (r2);
\draw[->, thick, bend right=13] (wp2) to (r4);
\draw[->, thick, bend right=20] (wp4) to (wp1);
\draw[->, thick, bend right=0] (w3) to (r5);
\draw[->, thick, bend right=0] (w4) to (r5);
\draw[->, thick, bend right=20] (wp5) to (wp3);
\draw[->, thick, bend right=0] (wp5) to (wp4);



\end{tikzpicture}
\caption{
The reduction to $\ROPosetRealizability$.
}
\label{subfig:rscrm_reduction2}
\end{subfigure}
\caption{
Example of our reduction of an instance of $\OPosetRealizability$ (\protect\ref{subfig:rscrm_reduction1}) to an instance of $\ROPosetRealizability$ (\protect\ref{subfig:rscrm_reduction2}) .
}
\label{fig:rscrm}
\end{figure}

==> linear_time_classes.tex <==
\section{Linear-time classes}\label{sec:linear_time}


\smallskip\noindent{\bf Trace spaces.}
Consider a trace $\Trace$ and an ideal $X$ of $\Trace$.
We define the \emph{trace space} of $X$ as a rooted tree $\Tree_X=(\TreeNodes_X, \TreeEdges_X)$, where 
$\TreeNodes_X$ is the set of nodes that consists of traces of events in $X$
and $\TreeEdges_X$ is the set of directed  edges.
In particular, the $\TreeNodes_X$ is the smallest set that satisfies the following properties.
\begin{compactenum}
\item We have $\epsilon\in \TreeNodes_X$.
\item For every $\Trace_1\in \TreeNodes_X$, we distinguish the following cases.
\begin{compactenum}
\item If there exists an event $\Event\in \Extend{X}{\Trace_1}$ such that either
(i)~there exists a pair $(\Write, \Event)\in \Frontier{X}{\Trace_1}$ (i.e., $\Event$ is a read event in the frontier of $\Trace_1$) or 
(ii)~there exists no pair $(\Event, \Read)\in \Frontier{X}{\Trace_1}$ (i.e., $\Event$ is not a write event in the frontier of $\Trace_1)$,
we choose such an event arbitrarily and construct the trace $\Trace_2=\Trace_1\circ \Event$.
We let $\Trace_2\in \TreeNodes_X$ and $(\Trace_1, \Trace_2)\in \TreeEdges_X$.
\item Otherwise, for every event $\Write\in \Enabled{X}{\Events{\Trace_1}}$, we construct the trace $\Trace_{\Write}=\Trace_1 \circ \Write$.
We let $\Trace_{\Write}\in \TreeNodes_X$ and $(\Trace_1, \Trace_{\Write})\in \TreeEdges_X$.
\end{compactenum}
\end{compactenum}

We have $\epsilon\in \TreeNodes_X$, and for every trace $\Trace_1\in \TreeNodes_X$ and event $\Event\in X$ such that $\Events{\Trace_1}$ is extensible with $\Event$, we have $\Trace_2=\Trace_1\circ \Event\in \TreeNodes_X$.
In this case, we have the directed edge $(\Trace_1, \Trace_2)\in \TreeEdges_X$, and $\Label_X(\Trace_1, \Trace_2)=\Event$.
We let $\epsilon$ be the root of $\Tree_X$.

Note that every trace $\Trace'\in \TreeNodes_X$ is a correct reordering of $\Trace$.
The trace space $\Tree_X$ is, in general, exponentially large.
However, here we identify cases where the race detection problem can be solved by exploring only linearly many nodes of $\Tree_X$.


\smallskip\noindent{\bf Accepting paths and accepting nodes.}
Consider a trace $\Trace$, an ideal $X$ of $\Trace$ and the trace space $\Tree_X$ of $X$.
A path $P$ is \emph{accepting} if the last node of $P$ is a trace $\Trace'$ such that $|\Trace'|=|X|$,
i.e., $\Trace'$ is a leaf of $\Tree_X$ that contains all events of $X$.
A node $\Trace'\in \TreeNodes_X$ is accepting there is an accepting path starting from $\Trace'$.
Finally, we say that $\Tree_X$ is accepting if the root of $\Tree_X$ is accepting.

\smallskip
\begin{remark}\label{rem:trace_space}
The ideal $X$ is realizable iff the trace space $\Tree_X$ is accepting.
\end{remark}


\input{constant_variables}
%\input{constant_remote_reads}
%\input{constant_context_switches}

==> np_hardness.tex <==
\subsection{Hardness of Data Race Prediction}\label{subsec:np_hardness}

Here we establish the NP-completeness of dynamic data race prediction.
Observe that membership in NP is straightforward, hence our focus is on showing NP-hardness.
Our reduction is based on the hardness of the realizability of o-posets.
For succinctness, we denote by $\OPosetRealizability$ the realizability problem of o-posets.

\smallskip
\begin{lemma}[{\cite[Theorem~4.1]{Gibbons97}}]\label{lem:oposet_hard}
$\OPosetRealizability$ is NP-complete.
\end{lemma}


Our proof of \cref{them:general_npc} is by a two-step reduction.
First we define a variant of the realizability problem for o-posets, namely $\ROPosetRealizability$, and show that it is NP-hard.
Afterwards, we reduce $\ROPosetRealizability$ to the dynamic data race prediction problem, which concludes the NP-hardness of the latter.
In this section, we assume wlog that for any o-poset $\OPoset=(X,P,\Observation)$, 
for each triplet $(\Write, \Read, \Write')\in \ReadTriplets{\OPoset}$, we have
$\Unordered{\Write'}{P}{\Write}$ and
$\Unordered{\Write'}{P}{\Read}$.
Given such a triplet $\sigma=(\Write, \Read, \Write')$, 
we refer to $\Write$, $\Read$ and $\Write'$ as the
\emph{write}, \emph{read}, and \emph{interfering write} event of $\sigma$, respectively.





\Paragraph{Reverse o-poset realizability.}
We define the problem $\ROPosetRealizability$ as follows.
We are given a tuple $(X,P,\Observation,\sigma,\Trace)$ where $\OPoset=(X,P,\Observation)$ is an o-poset,
$\sigma=(\ov{\Write}, \ov{\Read}, \ov{\Write}')$ is a distinguished triplet of $\OPoset$, 
and $\Trace$ is a witness to the realizability of $\OPoset$ such that $\ov{\Write}'<_{\Trace}\ov{\Write}$.
The task is to determine whether $\OPoset$ has a linearization $\Trace'$ such that $\ov{\Write}<_{\Trace'} \ov{\Write}'$,
i.e., the ordering between $\ov{\Write}$ and $\ov{\Write}'$ is reversed in $\Trace'$.


\Paragraph{Hardness of $\ROPosetRealizability$.}
We show that $\ROPosetRealizability$ is NP-hard by means of a reduction from $\OPosetRealizability$.
We first present the construction and then argue about its correctness.

\SubParagraph{Construction.}
Consider any instance $\OPoset=(X,P,\Observation)$ of $\OPosetRealizability$ and we construct an instance $\OPosetQ=(X',P', \Observation', \sigma, \Trace)$ of $\ROPosetRealizability$.
We assume wlog that $X$ contains only the events of the triplets of $\OPoset$ and for every such triplet $(\Write, \Read, \Write')$ we have $\Write<_{P} \Read$.
We show how to construct the o-poset $\OPosetS=(X',P', \Observation')$ by describing its set of triplets and the partial order $P'$.
\cref{fig:rscrm} provides an illustration.
Similarly to $\OPoset$, the set $X'$ contains all the events of the triplets of $\OPosetS$.
The key idea of the construction is that when we reverse the ordering in the distinguished triplet $\sigma$, the partial order $P$ coincides with the closure of $P'$ when projected to $X$.
The set $\ReadTriplets{\OPosetS}$ consists of the following triplets.
\begin{compactenum}
\item Every triplet $(\Write_i, \Read_i, \Write'_i)$ of $\OPoset$.
\item One triplet $(\Write_{\Event, \Event'}, \Read_{\Event, \Event'}, \Write_{\Event, \Event'}')$ for every two events $\Event, \Event'\in X$ such that $\Event<_{P}\Event'$.
\item One distinguished triplet $\sigma=(\ov{\Write}, \ov{\Read}, \ov{\Write}')$.
\end{compactenum}
The partial order $P'$ is constructed as follows.
For every triplet of $(\Write, \Read, \Write')$ of $\OPosetS$, we have
$\Write <_{P'}\Read$.
In addition, for every triplet of $\OPosetS$ of the form $(\Write_{\Event, \Event'}, \Read_{\Event, \Event'}, \Write_{\Event, \Event'}')$, we have
\begin{align*}
&\Event<_{P'}\Read_{\Event, \Event'}
\quad\text{and}\quad
\Write'_{\Event, \Event'}<_{P'}\Event'
\quad\text{and}\quad\\
&\Write_{\Event, \Event'}<_{P'} \ov{\Read}
\quad\text{and}\quad
\ov{\Write}'<_{P'} \Write'_{\Event, \Event'}
\end{align*}
The key idea of the construction is that for any closed partial order $Q\Refines P'$, if $\Read<_{Q} \Write'$ then $\Event<_{Q} \Event'$.
We next argue that $P'$ is indeed a partial order.

\smallskip
\begin{restatable}{lemma}{lemppo}\label{lem:p_po}
$P'$ is a partial order.
\end{restatable}
\begin{proof}
Assume towards contradiction otherwise, and consider any cycle $\Event_1 <_{P'} \Event_2<_{P'}\dots<_{P'} \Event_1$ in $P'$.
Let $C=\{ \Event_i\colon \Event_i \in X'\setminus X \}$, and note that that $C\neq \emptyset$, since no event in $X$ has an immediate successor in $X$ wrt $P'$.
Observe that no event $\Event_i\in C$ is the read event of some triplet of $\OPosetS$, as all such events are maximal in $P'$.
In addition, no event $\Event_i\in C$ is the write event of some triplet of $\OPosetS$, as the only successor of $\Event_i$ is the read event of the distinguished triplet $\sigma$, which has no successors.
Finally, no event $\Event_i\in C$ is the interfering write event of some triplet of $\OPosetS$, as the only predecessor of $\Event_i$ is $\ov{\Write}'$ (i.e., the interfering write event of the distinguished triplet $\sigma$), which in turn has no predecessors in $P'$.
Hence $C=\emptyset$, a contradiction.

The desired result follows.
\end{proof}

We now turn our attention to the solution $\Trace$ of $\OPosetS$, which is constructed in two steps.
First, we construct a partial order $Q\Refines P'$ over $X'$ such that for every triplet $(\Write,\Read,\Write')$ of $\OPosetS$, we have $\ov{\Write}' <_{Q}\ov{\Write}$.
Then, we obtain $\Trace$ by linearizing $Q$ arbitrarily.

\smallskip
\begin{restatable}{lemma}{lemwitness}\label{lem:witness}
The linearization $\Trace$ realizes $\OPosetS$.
\end{restatable}
\begin{proof}
We argue that $Q$ is indeed a partial order, from which follows that $\Trace$ is a witness of the realizability of $\OPosetS$.
Observe that the following hold by construction.
\begin{compactenum}
\item For any triplet $(\Write, \Read, \Write')$ of $\OPosetS$,
if for some $\Event\in X'$ we have $\Write<_{P'}\Event$,
then $\Event$ is the read event of some triplet in $\ReadTriplets{\OPosetS}\setminus\ReadTriplets{\OPoset}$.
\item Every read event of each triplet in $\ReadTriplets{\OPosetS}\setminus\ReadTriplets{\OPoset}$ is a maximal event in $P'$.
\end{compactenum}
Hence, in $Q$ we have $\Write \not<_{Q}\Write'$ for every two events $\Write$, $\Write'$, which are the write and interfering write event of some triplet of $\OPoset$, respectively.
Since we create $Q$ by ordering $\Write'<_{Q}\Write$, we have that no cycle is formed in $Q$.

The desired result follows.
\end{proof}

Observe that $\ROPosetRealizability$ has size polynomial in the size of $\OPosetRealizability$.
In the following lemma we prove the correctness of the above reduction, which concludes the hardness of $\ROPosetRealizability$.

\smallskip
\begin{restatable}{lemma}{lemrscrmhardness}\label{lem:rscrm_hardness}
$\ROPosetRealizability$ is NP-complete.
\end{restatable}
\begin{proof}

Membership in NP is straightforward.
Here we argue that $\OPoset$ has a witness $\Trace_1$ iff $\OPosetQ$ has a witness $\Trace_2$.

\noindent{\em $\Rightarrow$.}
Consider the witness $\Trace_1$ for $\OPoset$, and we show how to obtain the witness $\Trace_2$ for $\OPosetQ$.
We construct a partial order $Q$ over $X'$ such that
(i)~$Q\Refines P'$,
(ii)~for every triplet $(\Write, \Read, \Write')\in \ReadTriplets{\OPosetS}\setminus\ReadTriplets{\OPoset}$, we have $\Read <_{Q} \Write'$, and 
(iii)~$Q\Project X = \Trace_1$ (i.e., $Q$ totally orders the events of $X$ according to $\Trace_1$).
Afterwards, we construct $\Trace_2$ by linearizing $Q$ arbitrarily.
Note that (ii) makes $Q\Project X=P$, hence the linearization in (iii) is well defined.


\noindent{\em $\Leftarrow$.}
Consider the witness $\Trace_2$ for $\OPosetQ$, and we show how to obtain the witness $\Trace_1$ for $\OPoset$.
We construct $\Trace_1$ simply as $\Trace_1=\Trace_2 \Project X$.
To see that $\Trace_1$ is a linearization of $(X,P)$, consider any two events $\Event, \Event'\in X$ such that $\Event<_{P}\Event'$.
Consider the triplet $(\Write_{\Event, \Event'}, \Read_{\Event, \Event'}, \Write_{\Event, \Event'}')$ of $\OPosetQ$,
and we have $\Write_{\Event, \Event'}<_{\Trace_2}\Write'_{\Event, \Event'}$, thus $\Read_{\Event, \Event'}<_{\Trace_2}\Write'_{\Event, \Event'}$.
This leads to $\Event<_{\Trace_2}\Event'$, and thus $\Event<_{\Trace_1}\Event'$, as desired.



The desired result follows.
\end{proof}

\input{figures/fig_rscrm_reduction}


\Paragraph{Hardness of dynamic data race prediction.}
We are now ready to prove the second step of the reduction, i.e.,
reducing $\ROPosetRealizability$ to the decision problem of dynamic data race prediction.
We first describe the construction and then prove its correctness


Consider an instance $\OPosetS=(X,P, \Observation, \sigma, \Trace)$ of $\ROPosetRealizability$, and we construct a trace $\Trace'$ and two events $\Event_1, \Event_2\in \Events{\Trace'}$ such that $(\Event_1, \Event_2)$ is a predictable data race of $\Trace'$ iff $\OPosetS$ is realizable. We assume wlog that $X$ contains only events that appear in triplets of $\OPosetS$.
\cref{fig:race_reduction} provides an illustration.

Let $n=|\ReadTriplets{\OPosetS}|$.
We first construct an event set $X'$, a thread order $\TO$ and an observation function $\Observation': \ReadsReleases{X'}\to \WritesAcquires{X'}$.
Afterwards, we show how to construct the trace $\Trace'$ such that $\Events{\Trace'}=X'$, $\Trace'\Refines \TO$ and $\Observation_{\Trace'}=\Observation'$.
\begin{compactenum}
\item We have $k=2\cdot n$ threads $\{ \Process_i \}_{1\leq i\leq k}$. We introduce a variable $y$, a write event $\ov{\Write}$ and a read event $\ov{\Read}$ with $\Location{\ov{\Write}}=\Location{\ov{\Read}}=y$. Afterwards, we will be deciding the dynamic data race prediction problem for $\Trace'$ and the event pair $(\ov{\Write}, \ov{\Read})$.
\item We associate with every triplet $(\Write_i, \Read_i, \Write'_i)\in \ReadTriplets{\OPosetS}$ a unique global variable $x_i$ and have $\Proc{\Write_i}=\Proc{\Read_i}=\Process_i$, $\Proc{\Write'_i}=\Process_{n+i}$, and $\Write_i<_{\TO} \Read_i$.
Additionally, we make $\Observation'(\Read_i)=\Write_i$.
\item For the distinguished triplet $\sigma=(\Write, \Read, \Write')$, we make $\Read<_{\TO}\ov{\Read}$ and $\Write'<_{\TO} \ov{\Write}$.
\item For every two events $\Event, \Event'\in X$ such that $\Event<_{P}\Event'$, we introduce a unique global variable $x_{\Event, \Event'}$
and a write event and a read event $\Write_{\Event, \Event'}$ and $\Read_{\Event, \Event'}$, respectively, such that $\Location{\Write_{\Event, \Event'}}=\Location{\Read_{\Event, \Event'}}=x_{\Event, \Event'}$ and $\Observation'(\Read_{\Event, \Event'})=\Write_{\Event, \Event'}$.
In addition, we make $\Proc{\Write_{\Event, \Event'}}=\Proc{\Event}$ and $\Proc{\Read_{\Event, \Event'}}=\Proc{\Event'}$.
The thread order $\TO$ orders $\Write_{\Event, \Event'}$ right after $\Event$ and $\Read_{\Event, \Event'}$ right before $\Event'$.
\item For each thread $\Process_i\neq \Proc{\Write},\Proc{\Write'}$ (i.e., $\Process_i$ is not the thread of the events of the distinguished triplet), we introduce a unique global variable $x^i$ and a write event and a read event $\Write^i$ and $\Read^i$, respectively, such that $\Location{\Write^i}=\Location{\Read^i}=x^i$ and $\Observation'(\Read^i)=\Write^i$.
In addition, we make $\Proc{\Write^i}=\Process_i$ and $\Proc{\Read^i}=\Proc{\Write}$.
For every event $\Event$ already introduced in thread $\Process_i$, we make $\Event<_{\TO}\Write^i$.
Also, we make $\Read^i<_{\TO} \ov{\Read}$.
\item Let $\sigma=(\Write, \Read, \Write')$ be the distinguished triplet of $\OPosetS$.
We introduce a lock variable $\ell$ and two lock-acquire-release pairs $(\Acquire_i, \Release_i)_i$, for $i\in[2]$, on lock $\ell$.
We make $\Proc{\Acquire_1}=\Proc{\Release_1}=\Proc{\Read}$ and $\Proc{\Acquire_2}=\Proc{\Release_2}=\Proc{\Write'}$.
The critical section on $\Acquire_1$ contains only the read event $\Read$,
whereas the critical section on $\Acquire_2$ contains all other events of $\Proc{\Write'}$.
\end{compactenum}
Observe that in the above construction, every event $\Event\in X$ appears in $X'$.
Moreover, for every two events $\Event_1,\Event_2\in X$, we have $\Event_1<_{P} \Event_2$ iff $\Event_1<_{\TOO} \Event_2$.


The trace $\Trace'$ is constructed by linearizing $(X',\TO, \Observation')$ arbitrarily, such that the following conditions hold.
\begin{compactenum}
\item For every pair $(\Read, \Write)\in \Observation'$, we have $\Write<_{\Trace'} \Read$.
\item For every triplet $(\Write_i, \Read_i, \Write'_i)\in \ReadTriplets{\OPosetS}$, 
the pairs $(\Write_i,\Write'_i)$ and $(\Read_i, \Write'_i)$ are ordered in $\Trace'$ as in $\Trace$.
\item Note that the previous item orders $\Write<_{\Trace'}\Write'$, for the distinguished triplet $\sigma=(\Write, \Read, \Write')$.
We also order $\Release_2<_{\Trace'}\Acquire_1$.
\end{compactenum}
Note that $\Trace'$ has size that is polynomial in $n$.
We conclude with the correctness proof of the above reduction, which concludes the lower bound of \cref{them:general_npc}.

\input{figures/fig_race_reduction}








\begin{proof}[Proof of \cref{them:general_npc}.]
Membership in NP is straightforward.
Here we show that $\OPosetS$ has a witness $\Trace_1$ iff $(\ov{\Write}, \ov{\Read})$ is a predictable data race of $\Trace'$, witnessed by a trace $\Trace_2$.

\noindent{\em $\Rightarrow$.}
Consider the witness $\Trace_1$, hence $\Read<_{\Trace_1}\Write'$ for the distinguished triplet $\sigma=(\Write, \Read, \Write')$.
The witness trace $\Trace_2$ is constructed such that 
(i)~$\Events{\Trace_2}=X'\setminus\{ \Release_2, \ov{\Write}, \ov{\Read} \}$,
(ii)~$\Release_1<_{\Trace_2}\Acquire_2$, and
(iii)~for every two events $\Event_1,\Event_2\in X$, we have $\Event_1<_{\Trace_2}\Event_1$ iff $\Event_1<_{\Trace_1}\Event_2$.
It follows easily that $\Trace_2$ is a linearization of the canonical o-poset of the trace ideal $X'\setminus \{ \Release_2, \ov{\Write}, \ov{\Read}\}$ of $\Trace'$.
Since $\ov{\Write}$, $\ov{\Read}$ are enabled in $\Trace_2$, we have that $\Trace_2$ is a witness of the data race $(\ov{\Write}, \ov{\Read})$.


\noindent{\em $\Leftarrow$.}
Consider the witness $\Trace_2$, and it is straightforward that $\Events{\Trace_2} = X'\setminus \{ \Release_2 , \ov{\Write}, \ov{\Read} \}$.
Hence $\Release_1<_{\Trace_2}\Acquire_2$ and thus $\Read<\Write'$ for the distinguished triplet $\sigma=(\Write, \Read, \Write')$.
The witness $\Trace_1$ is constructed such that for every two events $\Event_1, \Event_2\in X$, we have $\Event_1<_{\Trace_1}\Event_2$ iff $\Event_1<_{\Trace_2}\Event_2$.
It follows easily that $\Trace_1$ is a linearization of the o-poset $(X,P,\Observation)$ and $\Read<_{\Trace_1}\Write'$.
\end{proof}



